A computationally efficient reconstruction algorithm for circular cone-beam computed tomography using shallow neural networks

Circular cone-beam (CCB) Computed Tomography (CT) has become an integral part of industrial quality control, materials science and medical imaging. The need to acquire and process each scan in a short time naturally leads to trade-offs between speed and reconstruction quality, creating a need for fast reconstruction algorithms capable of creating accurate reconstructions from limited data. In this paper we introduce the Neural Network Feldkamp-Davis-Kress (NN-FDK) algorithm. This algorithm adds a machine learning component to the FDK algorithm to improve its reconstruction accuracy while maintaining its computational efficiency. Moreover, the NN-FDK algorithm is designed such that it has low training data requirements and is fast to train. This ensures that the proposed algorithm can be used to improve image quality in high throughput CT scanning settings, where FDK is currently used to keep pace with the acquisition speed using readily available computational resources. We compare the NN-FDK algorithm to two standard CT reconstruction algorithms and to two popular deep neural networks trained to remove reconstruction artifacts from the 2D slices of an FDK reconstruction. We show that the NN-FDK reconstruction algorithm is substantially faster in computing a reconstruction than all the tested alternative methods except for the standard FDK algorithm and we show it can compute accurate CCB CT reconstructions in cases of high noise, a low number of projection angles or large cone angles. Moreover, we show that the training time of an NN-FDK network is orders of magnitude lower than the considered deep neural networks, with only a slight reduction in reconstruction accuracy.

==> packages.tex <==
% !TEX root = paper.tex

%%%%%%%%%%%%
% Packages %
%%%%%%%%%%%%

%% Page Layout
%\usepackage{fullpage} %http://en.wikibooks.org/wiki/LaTeX/Page_Layout
% Manual headings and margins:
%\usepackage[activate=normal]{pdfcprot} % Textrï¿½nder werden einheitlicher angepasst, glatter Rand --> deprecated !!!
%\usepackage{fancyhdr}        % definiere einfache Headings
%\usepackage{float}
%\usepackage{vmargin}         % Seitenrï¿½nder einstellen leichtgemacht
%\usepackage[width=1cm, left=3cm]{geometry} % Alternative fï¿½r Seitenrï¿½nder
%\usepackage[Bjornstrup]{fncychap}       % Fancy Chapter Headings


%% Affliations
%\usepackage[affil-it]{authblk}%


%% PDF properties
%\usepackage[pagebackref,pdftex,bookmarks,colorlinks,breaklinks]{hyperref}
%% Define properties for the hyperref package
%%\hypersetup{%
%		%colorlinks=true,       %default: false
%		linkcolor=magenta,      %has effects if colorlinks=true
%		citecolor=blue,				
%		filecolor=dullmagenta,
%		urlcolor=magenta,
%		%menucolor=blue,
%		%plainpages=false,
%		%pdfpagemode=none,      %Alternative: =FullScreen
%		%pdfview=FitV,
%		%pdfstartview=FitH,
%		%pdffitwindow=true,
%		%pdfmenubar=false,      %default true
%		%pdfwindowui=false,     %default true
%		%bookmarksopen=true,
%		%bookmarksnumbered=true,
%		%bookmarksopenlevel=2,
%}



\makeatother
\usepackage{calc}  

%% AMS Latex packages
\usepackage{amsmath,amstext,amsfonts,amssymb,amsthm,latexsym}
\newtheorem{thm}{Theorem}
\newtheorem{mydef}{Definition}
\newtheorem{algo}{Algorithm}
\newtheorem{prop}{Proposition}
\usepackage{xfrac}
\usepackage{mathtools}
\mathtoolsset{showonlyrefs}
\usepackage{algorithmic}
\usepackage{lscape}
\usepackage{graphicx}
\usepackage{color}
% \usepackage{epstopdf}
% \usepackage{caption}
% \usepackage{subcaption}
\usepackage{rotating}
\usepackage{multimedia}
\usepackage{multicol}
\usepackage{mathtools}




%% Font packages
% \usepackage[latin1]{inputenc} % Definition des Eingabeencodings, also wie Umlaute umgesetzt werden
% \usepackage[T1]{fontenc}      % Zeichensatzkodierung T1
% \usepackage{ae}               % Verwendung von AE-Fonts
%\usepackage[german,ngerman]{babel}
% \usepackage{color}
%\definecolor{myred}{rgb}{0.695,0.148,0}
%\definecolor{mygray}{gray}{0.6}



% Additional symbols:
%\usepackage{wasysym}
%\usepackage{dsfont}          % Mathematische Zeichen wie R oder C mit Doppelstrichen 


%% TODO notes
%\usepackage{todonotes}


%% Figures
\usepackage{graphicx}         % for using includegraphics
\usepackage{epsfig}           % for using epsfig <-- uses includegraphics
%\usepackage{subfigure}
\usepackage{caption,subcaption} % http://en.wikibooks.org/wiki/LaTeX/Floats,_Figures_and_Captions
% \usepackage{sidecap}
% \usepackage{placeins}

%% Tables
%\usepackage{longtable}       % seitenï¿½bergreifende Tabellen
%\usepackage{array}           % fuer aufwï¿½ndigere Tabellen
%\usepackage{tabularx}        % tables with fixed col width and row height
%\usepackage{colortbl}        % farbige Tabellen (v. D. Carlisle)
%\usepackage{enumerate,enumitem,multirow,multicol}


%% Code visualization
%\usepackage{listings}        % fuer die Code-Umgebung
% algorithmicx packages:
%\usepackage{algorithm}
\usepackage{algorithm2e}
%\usepackage{algpseudocode}
%\usepackage{algorithmic}
%\usepackage[ruled,vlined]{algorithm2e} % do this BEFORE loading algorithmicx
\newenvironment{Model1}[1][htb]
  {\renewcommand{\algorithmcfname}{Model}% Update algorithm name
   \begin{algorithm}[#1]%
  }{\end{algorithm}}


%% Misc
%\usepackage[T1]{url}         % T1: allow line breaks for URLs
%\usepackage{acronym}         % Acronyms
%\usepackage{times}
%\usepackage{pgf,pgfarrows,pgfnodes,pgfautomata,pgfheaps} %Pfeile ?
%\usepackage{background}
%\usepackage{ifthen}
%\usepackage[rflt]{floatflt}
%\usepackage{cancel}			 % fuer Durchstreichungen
%\usepackage{bbm} ?


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Diagrams
%\usepackage{tikz}
%\usetikzlibrary{calc,trees,positioning,arrows,chains,shapes.geometric,%
%    decorations.pathreplacing,decorations.pathmorphing,shapes,%
%    matrix,shapes.symbols}
%\tikzset{
%	>=stealth',
%  element1/.style={
%    rectangle, 
%    rounded corners, 
%    % fill=black!10,
%    draw=black,% thick,
%    text width=10em,
%    minimum height=3em,
%    text centered, 
%    on chain},   
%%   line/.style={draw, thick, <->},
%%  element2/.style={
%%    tape,
%%    top color=white,
%%    bottom color=blue!50!black!60!,
%%    minimum width=8em,
%%    draw=blue!40!black!90, very thick,
%%    text width=10em, 
%%    minimum height=3.5em, 
%%    text centered, 
%%    on chain},
%  every join/.style={->, shorten >=1pt, shorten <=1pt,},% thick},
%  %decoration={brace},
%  %tuborg/.style={decorate},
%  %tubnode/.style={midway, right=2pt},
%}

